A Comprehensive Evaluation of Tool-Assisted Generation Strategies

A growing area of research investigates augmenting language models with tools (e.g., search engines, calculators) to overcome their shortcomings (e.g., missing or incorrect knowledge, incorrect logical inferences). Various few-shot tool-usage strategies have been proposed. However, there is no systematic and fair comparison across different strategies, or between these strategies and strong baselines that do not leverage tools. We conduct an extensive empirical analysis, finding that (1) across various datasets, example difficulty levels, and models, strong no-tool baselines are competitive to tool-assisted strategies, implying that effectively using tools with in-context demonstrations is a difficult unsolved problem; (2) for knowledge-retrieval tasks, strategies that *refine* incorrect outputs with tools outperform strategies that retrieve relevant information *ahead of* or *during generation*; (3) tool-assisted strategies are expensive in the number of tokens they require to work -- incurring additional costs by orders of magnitude -- which does not translate into significant improvement in performance. Overall, our findings suggest that few-shot tool integration is still an open challenge, emphasizing the need for comprehensive evaluations of future strategies to accurately assess their *benefits* and *costs*.

==> tables/results.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{[automatically generated]}\label{tab: }
\footnotesize
\begin{tabular}{lrrrrrrrr}\toprule
tool &sample &model &drop &gsm8k &musique\_em &musique\_f1 &strategy\_qa \\\midrule
Non-TA-Toolformer &3-2-1 &Flan-PaLM-540B &77.8 &69.8 &20.8 &30.39 &71.62 \\
Non-TA-Toolformer &mixshot\_max &Flan-PaLM-540B &77.8 &72.6 &20.8 &31.19 &79.91 \\
Non-TA-CoT &3-2-1 &Flan-PaLM-540B &77.2 &67.4 &21.6 &33.07 &79.91 \\
Non-TA-CoT &mixshot\_max &Flan-PaLM-540B &77.2 &70.8 &22.4 &33.80 &84.28 \\
Toolformer &3-2-1 &Flan-PaLM-540B &76.2 &61.2 &19.4 &31.89 &70.31 \\
Toolformer &mixshot\_max &Flan-PaLM-540B &76.2 &70.8 &20.6 &32.39 &73.36 \\
RnR &3-2-1 &Flan-PaLM-540B &76.0 &68.4 &20.4 &30.53 &79.91 \\
RnR &mixshot\_max &Flan-PaLM-540B &76.0 &70.4 &22.8 &33.48 &80.79 \\
Non-TA-Toolformer &mixshot\_avg &Flan-PaLM-540B &75.9 &71.2 &20.2 &30.77 &74.67 \\
Non-TA-Toolformer &2-1-5-7-4 &Flan-PaLM-540B &75.6 &72.6 &20.0 &30.71 &79.91 \\
Non-TA-CoT &mixshot\_avg &Flan-PaLM-540B &75.5 &69.7 &21.9 &33.41 &82.10 \\
Toolformer &mixshot\_avg &Flan-PaLM-540B &75.3 &64.5 &19.9 &32.05 &72.20 \\
Toolformer &2-1-5-7-4 &Flan-PaLM-540B &75.2 &61.4 &20.6 &32.39 &72.93 \\
Non-TA-CoT &2-1-5-7-4 &Flan-PaLM-540B &75.0 &70.8 &21.6 &33.36 &84.28 \\
Toolformer &5-3-6-1-4-0-2 &Flan-PaLM-540B &74.4 &70.8 &19.6 &31.88 &73.36 \\
Non-TA-Toolformer &5-3-6-1-4-0-2 &Flan-PaLM-540B &74.4 &71.2 &19.8 &31.19 &72.49 \\
Non-TA-CoT &5-3-6-1-4-0-2 &Flan-PaLM-540B &74.2 &70.8 &22.4 &33.80 &82.10 \\
RnR &2-1-5-7-4 &Flan-PaLM-540B &73.6 &70.4 &21.6 &32.97 &80.79 \\
Non-TA-Toolformer &2-1-5-7-4 &GPT-3 &66.0 &54.0 &14.8 &30.33 &75.98 \\
Non-TA-Toolformer &mixshot\_max &GPT-3 &66.0 &54.0 &15.2 &30.33 &78.60 \\
Toolformer &2-1-5-7-4 &GPT-3 &66.0 &52.4 &20.4 &36.65 &72.05 \\
Toolformer &mixshot\_max &GPT-3 &66.0 &52.8 &20.4 &36.65 &72.05 \\
Non-TA-CoT &3-2-1 &Flan-PaLM-62B &65.6 &47.4 &12.0 &23.60 &75.98 \\
Non-TA-CoT &mixshot\_max &Flan-PaLM-62B &65.6 &47.4 &12.0 &24.27 &80.35 \\
RnR &3-2-1 &Flan-PaLM-62B &65.0 &46.8 &14.4 &25.21 &75.55 \\
RnR &mixshot\_max &Flan-PaLM-62B &65.0 &46.8 &16.0 &26.47 &76.42 \\
RnR &mixshot\_avg &Flan-PaLM-540B &64.9 &69.7 &21.6 &32.33 &79.62 \\
Non-TA-Toolformer &2-1-5-7-4 &Flan-PaLM-62B &64.0 &47.8 &11.8 &22.69 &73.36 \\
Non-TA-Toolformer &mixshot\_max &Flan-PaLM-62B &64.0 &48.8 &12.8 &23.42 &75.55 \\
Toolformer &2-1-5-7-4 &Flan-PaLM-62B &64.0 &47.8 &2.6 &11.65 &63.32 \\
Toolformer &mixshot\_max &Flan-PaLM-62B &64.0 &48.8 &6.2 &12.52 &63.32 \\
Non-TA-CoT &2-1-5-7-4 &Flan-PaLM-62B &63.6 &46.2 &11.4 &23.42 &79.04 \\
RnR &2-1-5-7-4 &Flan-PaLM-62B &63.6 &44.0 &16.0 &26.39 &71.18 \\
Non-TA-CoT &mixshot\_avg &Flan-PaLM-62B &62.8 &47.0 &11.6 &23.76 &78.46 \\
Non-TA-Toolformer &mixshot\_avg &GPT-3 &61.1 &52.9 &14.7 &29.20 &74.96 \\
Non-TA-Toolformer &mixshot\_avg &Flan-PaLM-62B &60.7 &48.2 &11.9 &22.66 &74.67 \\
Non-TA-Toolformer &5-3-6-1-4-0-2 &GPT-3 &59.6 &53.2 &14.0 &28.15 &78.60 \\
Toolformer &mixshot\_avg &Flan-PaLM-62B &59.6 &48.3 &3.7 &11.57 &62.01 \\
Non-TA-CoT &5-3-6-1-4-0-2 &Flan-PaLM-62B &59.2 &47.4 &11.4 &24.27 &80.35 \\
Non-TA-Toolformer &5-3-6-1-4-0-2 &Flan-PaLM-62B &59.2 &48.0 &11.0 &21.86 &75.55 \\
Non-TA-Toolformer &3-2-1 &Flan-PaLM-62B &59.0 &48.8 &12.8 &23.42 &75.11 \\
Toolformer &5-3-6-1-4-0-2 &Flan-PaLM-62B &57.8 &48.2 &2.2 &10.55 &61.57 \\
RnR &mixshot\_avg &Flan-PaLM-62B &57.6 &45.8 &15.4 &26.02 &74.38 \\
Non-TA-CoT &3-2-1 &GPT-3 &57.6 &58.8 &14.8 &27.37 &70.74 \\
Non-TA-CoT &mixshot\_max &GPT-3 &57.6 &58.8 &16.0 &30.25 &71.62 \\
Non-TA-Toolformer &3-2-1 &GPT-3 &57.6 &51.6 &15.2 &29.11 &70.31 \\
Toolformer &3-2-1 &Flan-PaLM-62B &57.0 &48.8 &6.2 &12.52 &61.14 \\
Toolformer &3-2-1 &GPT-3 &56.8 &50.8 &19.6 &34.90 &70.31 \\
Non-TA-CoT &mixshot\_avg &GPT-3 &56.3 &58.4 &15.3 &28.98 &71.32 \\
Toolformer &mixshot\_avg &GPT-3 &56.0 &52.0 &19.1 &34.29 &70.89 \\
Non-TA-CoT &2-1-5-7-4 &GPT-3 &55.6 &58.0 &15.2 &29.31 &71.62 \\
Non-TA-CoT &5-3-6-1-4-0-2 &GPT-3 &55.6 &58.4 &16.0 &30.25 &71.62 \\
RnR &3-2-1 &GPT-3 &54.8 &56.0 &18.4 &29.66 &72.05 \\
RnR &5-3-6-1-4-0-2 &GPT-3 &54.8 &61.6 &18.4 &32.26 &70.74 \\
RnR &mixshot\_max &GPT-3 &54.8 &61.6 &21.6 &32.95 &73.80 \\
RnR &mixshot\_avg &GPT-3 &54.7 &58.7 &19.5 &31.62 &72.20 \\
RnR &2-1-5-7-4 &GPT-3 &54.4 &58.4 &21.6 &32.95 &73.80 \\
Toolformer &5-3-6-1-4-0-2 &GPT-3 &45.2 &52.8 &17.2 &31.32 &70.31 \\
RnR &5-3-6-1-4-0-2 &Flan-PaLM-540B &45.0 &70.2 &22.8 &33.48 &78.17 \\
RnR &5-3-6-1-4-0-2 &Flan-PaLM-62B &44.2 &46.6 &15.8 &26.47 &76.42 \\
Non-TA-CoT &2-1-5-7-4 &Flan-UL2-20B &12.6 &27.2 &7.8 &16.50 &71.62 \\
Non-TA-Toolformer &2-1-5-7-4 &Flan-UL2-20B &9.2 &5.6 &4.6 &13.33 &68.56 \\
Non-TA-Toolformer &mixshot\_max &Flan-UL2-20B &9.2 &5.6 &5.0 &13.66 &72.05 \\
Non-TA-Toolformer &mixshot\_avg &Flan-UL2-20B &4.2 &4.3 &4.2 &12.24 &70.60 \\
Non-TA-Toolformer &3-2-1 &Flan-UL2-20B &2.6 &3.6 &5.0 &13.66 &72.05 \\
Non-TA-CoT &5-3-6-1-4-0-2 &Flan-UL2-20B &0.8 &26.2 &7.2 &16.10 &72.05 \\
Non-TA-Toolformer &5-3-6-1-4-0-2 &Flan-UL2-20B &0.8 &3.6 &3.0 &9.74 &71.18 \\
RARR-Top5 &mixshot\_avg &Flan-PaLM-540B & & &24.4 &35.65 &80.06 \\
RARR &mixshot\_avg &Flan-PaLM-540B & & &23.2 &34.70 &80.64 \\
Toolformer-Top5 &mixshot\_avg &Flan-PaLM-540B & & &21.2 &32.97 &72.05 \\
RnR-Top5 &mixshot\_avg &Flan-PaLM-540B & & &22.1 &32.76 &80.49 \\
RnR-Top5 &2-1-5-7-4 &Flan-PaLM-540B & & &21.6 &32.68 &81.66 \\
RnR-Top5 &5-3-6-1-4-0-2 &Flan-PaLM-540B & & &23.4 &33.87 &81.22 \\
RARR &2-1-5-7-4 &Flan-PaLM-540B & & &23.2 &35.09 &81.22 \\
RARR &5-3-6-1-4-0-2 &Flan-PaLM-540B & & &23.0 &34.14 &80.79 \\
RARR-Top5 &3-2-1 &Flan-PaLM-540B & & &25.0 &36.12 &80.35 \\
RARR-Top5 &2-1-5-7-4 &Flan-PaLM-540B & & &23.8 &35.40 &79.91 \\
RARR-Top5 &5-3-6-1-4-0-2 &Flan-PaLM-540B & & &24.4 &35.44 &79.91 \\
RARR &3-2-1 &Flan-PaLM-540B & & &23.4 &34.86 &79.91 \\
RnR-Top5 &3-2-1 &Flan-PaLM-540B & & &21.4 &31.74 &78.60 \\
Non-TA-CoT &mixshot\_avg &Flan-UL2-20B & &20.2 &7.0 &15.91 &70.31 \\
RARR &mixshot\_avg &Flan-PaLM-62B & & &11.5 &23.70 &77.15 \\
RARR &mixshot\_max &Flan-PaLM-540B & & &23.4 &35.09 &81.22 \\
RARR &mixshot\_max &Flan-UL2-20B & & &4.8 &13.40 &55.90 \\
RARR &mixshot\_max &Flan-PaLM-62B & & &12.0 &24.07 &77.73 \\
Interleave &2-1-5-7-4 &Flan-PaLM-540B & & &13.0 &21.29 &78.17 \\
Toolformer &mixshot\_avg &Flan-UL2-20B & &26.3 &6.8 &12.52 &66.08 \\
Non-TA-CoT &mixshot\_max &Flan-UL2-20B & &27.2 &7.8 &16.50 &72.05 \\
Toolformer-Top5 &2-1-5-7-4 &Flan-PaLM-540B & & &22.6 &34.53 &77.73 \\
RARR &2-1-5-7-4 &Flan-PaLM-62B & & &11.4 &23.42 &77.73 \\
RARR &5-3-6-1-4-0-2 &Flan-PaLM-62B & & &11.2 &24.07 &77.73 \\
Non-TA-SelfAsk &3-2-1 &Flan-PaLM-540B & & &18.6 &25.80 &76.86 \\
Interleave &3-2-1 &Flan-PaLM-540B & & &15.0 &23.71 &76.86 \\
RARR-Top5 &3-2-1 &Flan-PaLM-62B & & &12.0 &23.60 &75.98 \\
RARR &3-2-1 &Flan-PaLM-62B & & &12.0 &23.60 &75.98 \\
Non-TA-SelfAsk &2-1-5-7-4 &Flan-PaLM-62B & & &5.2 &9.52 &75.98 \\
Interleave &5-3-6-1-4-0-2 &Flan-PaLM-540B & & &12.4 &20.51 &75.98 \\
Non-TA-SelfAsk &5-3-6-1-4-0-2 &Flan-PaLM-540B & & &17.2 &24.31 &75.55 \\
SelfAskQA &5-3-6-1-4-0-2 &Flan-PaLM-540B & & &13.2 &22.81 &75.11 \\
Toolformer-Search &5-3-6-1-4-0-2 &Flan-PaLM-540B & & &14.0 &22.87 &74.67 \\
SelfAskQA &mixshot\_avg &GPT-3 & & &17.5 &31.46 &67.83 \\
RnR &mixshot\_avg &Flan-UL2-20B & &24.1 &5.1 &12.06 &60.99 \\
Toolformer-Search &mixshot\_avg &GPT-3 & & &17.7 &31.14 &69.43 \\
Non-TA-SelfAsk &mixshot\_avg &Flan-PaLM-62B & & &3.9 &6.74 &69.72 \\
Non-TA-SelfAsk &mixshot\_max &Flan-PaLM-540B & & &18.6 &25.80 &76.86 \\
Non-TA-SelfAsk &mixshot\_max &Flan-UL2-20B & & &4.6 &11.52 &53.71 \\
Non-TA-SelfAsk &mixshot\_max &GPT-3 & & &15.6 &29.80 &74.24 \\
Non-TA-SelfAsk &mixshot\_max &Flan-PaLM-62B & & &5.2 &9.52 &75.98 \\
Interleave &3-2-1 &Flan-PaLM-62B & & &15.6 &23.43 &74.67 \\
Interleave &5-3-6-1-4-0-2 &Flan-PaLM-62B & & &17.0 &24.42 &74.67 \\
Toolformer-Search &3-2-1 &Flan-PaLM-540B & & &10.4 &18.89 &74.24 \\
SelfAsk &5-3-6-1-4-0-2 &Flan-PaLM-540B & & &13.6 &23.36 &74.24 \\
Non-TA-SelfAsk &2-1-5-7-4 &GPT-3 & & &12.8 &28.13 &74.24 \\
Non-TA-SelfAsk &5-3-6-1-4-0-2 &Flan-PaLM-62B & & &3.2 &5.43 &74.24 \\
Toolformer-Search &2-1-5-7-4 &Flan-PaLM-540B & & &15.0 &24.27 &73.80 \\
Non-TA-SelfAsk &5-3-6-1-4-0-2 &GPT-3 & & &15.6 &29.80 &73.36 \\
Non-TA-SelfAsk &2-1-5-7-4 &Flan-PaLM-540B & & &16.8 &25.34 &73.36 \\
Toolformer-Top5 &5-3-6-1-4-0-2 &Flan-PaLM-540B & & &20.4 &31.69 &72.93 \\
Interleave &2-1-5-7-4 &Flan-PaLM-62B & & &16.0 &23.71 &72.49 \\
SelfAskQA-Top5 &5-3-6-1-4-0-2 &Flan-PaLM-540B & & &12.2 &21.99 &72.05 \\
Toolformer-Search &mixshot\_avg &Flan-UL2-20B & & &8.2 &14.80 &48.76 \\
SelfAsk &mixshot\_avg &Flan-PaLM-62B & & &8.1 &13.76 &67.10 \\
SelfAsk &mixshot\_max &Flan-PaLM-540B & & &14.2 &23.40 &74.24 \\
SelfAsk &mixshot\_max &Flan-UL2-20B & & &3.6 &11.86 &49.78 \\
SelfAsk &mixshot\_max &GPT-3 & & &12.8 &24.38 &67.25 \\
SelfAsk &mixshot\_max &Flan-PaLM-62B & & &9.0 &14.80 &67.69 \\
Non-TA-SelfAsk &3-2-1 &GPT-3 & & &12.8 &27.98 &72.05 \\
SelfAskQA &3-2-1 &Flan-PaLM-540B & & &12.4 &21.08 &71.62 \\
SelfAsk &3-2-1 &Flan-PaLM-540B & & &11.4 &20.02 &71.62 \\
Toolformer &3-2-1 &Flan-UL2-20B & &26.6 &10.2 &18.07 &71.18 \\
SelfAsk &2-1-5-7-4 &Flan-PaLM-540B & & &14.2 &23.40 &70.74 \\
Toolformer-Search &3-2-1 &GPT-3 & & &16.8 &28.85 &70.31 \\
Toolformer-Search &5-3-6-1-4-0-2 &Flan-PaLM-62B & & &7.0 &13.32 &70.31 \\
Toolformer &2-1-5-7-4 &Flan-UL2-20B & &26.2 &10.0 &17.94 &70.31 \\
SelfAskQA-Top5 &2-1-5-7-4 &Flan-PaLM-540B & & &12.6 &21.60 &70.31 \\
SelfAskQA &5-3-6-1-4-0-2 &GPT-3 & & &16.8 &30.34 &70.31 \\
SelfAskQA-Top5 &3-2-1 &Flan-PaLM-540B & & &11.0 &19.75 &69.87 \\
RnR &5-3-6-1-4-0-2 &Flan-UL2-20B & &23.2 &5.6 &13.52 &69.87 \\
RARR &mixshot\_avg &Flan-UL2-20B & & &4.5 &12.80 &46.29 \\
Non-TA-SelfAsk &mixshot\_avg &GPT-3 & & &13.7 &28.64 &73.22 \\
SelfAskQA &mixshot\_avg &Flan-PaLM-62B & & &10.9 &15.81 &68.12 \\
SelfAskQA &mixshot\_max &Flan-PaLM-540B & & &13.2 &22.81 &75.11 \\
SelfAskQA &mixshot\_max &Flan-UL2-20B & & &3.2 &8.53 &47.16 \\
SelfAskQA &mixshot\_max &GPT-3 & & &18.0 &32.74 &70.31 \\
SelfAskQA &mixshot\_max &Flan-PaLM-62B & & &12.6 &17.49 &69.00 \\
Toolformer-Search &2-1-5-7-4 &GPT-3 & & &17.6 &31.03 &69.43 \\
SelfAskQA &5-3-6-1-4-0-2 &Flan-PaLM-62B & & &10.0 &14.51 &69.00 \\
SelfAskQA &2-1-5-7-4 &Flan-PaLM-540B & & &12.8 &21.92 &69.00 \\
Non-TA-SelfAsk &mixshot\_avg &Flan-UL2-20B & & &3.7 &11.48 &45.41 \\
Toolformer &mixshot\_max &Flan-UL2-20B & &26.6 &10.2 &18.07 &71.18 \\
Toolformer-Search &5-3-6-1-4-0-2 &GPT-3 & & &18.8 &33.54 &68.56 \\
Toolformer-Search &2-1-5-7-4 &Flan-PaLM-62B & & &4.4 &9.45 &68.56 \\
SelfAskQA &2-1-5-7-4 &Flan-PaLM-62B & & &12.6 &17.49 &68.12 \\
SelfAsk &mixshot\_avg &Flan-UL2-20B & & &2.9 &8.98 &32.90 \\
RnR &mixshot\_max &Flan-UL2-20B & &25.8 &5.6 &13.52 &69.87 \\
SelfAskQA &2-1-5-7-4 &GPT-3 & & &17.6 &31.30 &67.69 \\
SelfAsk &2-1-5-7-4 &Flan-PaLM-62B & & &9.0 &14.80 &67.69 \\
SelfAskQA &3-2-1 &Flan-PaLM-62B & & &10.0 &15.42 &67.25 \\
SelfAsk &2-1-5-7-4 &GPT-3 & & &12.8 &24.15 &67.25 \\
SelfAsk &3-2-1 &Flan-PaLM-62B & & &7.8 &13.79 &67.25 \\
Non-TA-CoT &3-2-1 &Flan-UL2-20B & &7.2 &6.0 &15.14 &67.25 \\
SelfAskQA-Top5 &3-2-1 &Flan-PaLM-62B & & &11.6 &17.80 &66.81 \\
SelfAsk &5-3-6-1-4-0-2 &Flan-PaLM-62B & & &7.4 &12.68 &66.38 \\
SelfAsk &5-3-6-1-4-0-2 &GPT-3 & & &12.0 &22.33 &65.94 \\
Toolformer-Top5 &3-2-1 &Flan-PaLM-540B & & &20.6 &32.67 &65.50 \\
SelfAskQA &3-2-1 &GPT-3 & & &18.0 &32.74 &65.50 \\
SelfAsk &3-2-1 &GPT-3 & & &12.8 &24.38 &64.19 \\
Non-TA-SelfAsk &mixshot\_avg &Flan-PaLM-540B & & &17.5 &25.15 &75.25 \\
SelfAskQA &mixshot\_avg &Flan-UL2-20B & & &1.7 &5.39 &25.33 \\
SelfAsk &mixshot\_avg &GPT-3 & & &12.5 &23.62 &65.79 \\
Toolformer-Search &mixshot\_avg &Flan-PaLM-62B & & &5.5 &10.91 &64.48 \\
Toolformer-Search &mixshot\_max &Flan-PaLM-540B & & &15.0 &24.27 &74.67 \\
Toolformer-Search &mixshot\_max &Flan-UL2-20B & & &8.8 &14.93 &52.84 \\
Toolformer-Search &mixshot\_max &GPT-3 & & &18.8 &33.54 &70.31 \\
Toolformer-Search &mixshot\_max &Flan-PaLM-62B & & &7.0 &13.32 &70.31 \\
Toolformer-Top5 &3-2-1 &Flan-PaLM-62B & & &5.0 &11.74 &61.14 \\
RnR &2-1-5-7-4 &Flan-UL2-20B & &25.8 &5.4 &11.77 &60.70 \\
Non-TA-SelfAsk &3-2-1 &Flan-PaLM-62B & & &3.2 &5.28 &58.95 \\
Toolformer &5-3-6-1-4-0-2 &Flan-UL2-20B & &26.0 &0.2 &1.56 &56.77 \\
RARR &3-2-1 &Flan-UL2-20B & & &4.6 &13.40 &55.90 \\
Toolformer-Search &3-2-1 &Flan-PaLM-62B & & &5.2 &9.95 &54.59 \\
Non-TA-SelfAsk &5-3-6-1-4-0-2 &Flan-UL2-20B & & &3.6 &11.52 &53.71 \\
Toolformer-Search &2-1-5-7-4 &Flan-UL2-20B & & &8.8 &14.93 &52.84 \\
RnR &3-2-1 &Flan-UL2-20B & &23.2 &4.4 &10.90 &52.40 \\
SelfAsk &mixshot\_avg &Flan-PaLM-540B & & &13.1 &22.26 &72.20 \\
Interleave &mixshot\_avg &Flan-UL2-20B & & & & & \\
Interleave &mixshot\_avg &Flan-PaLM-62B & & &16.2 &23.85 &73.94 \\
Interleave &mixshot\_max &Flan-PaLM-540B & & &15.0 &23.71 &78.17 \\
Interleave &mixshot\_max &Flan-UL2-20B & & & & &0.00 \\
Interleave &mixshot\_max &Flan-PaLM-62B & & &17.0 &24.42 &74.67 \\
SelfAsk &3-2-1 &Flan-UL2-20B & & &3.6 &11.86 &49.78 \\
Toolformer-Search &3-2-1 &Flan-UL2-20B & & &8.4 &14.70 &48.47 \\
Non-TA-SelfAsk &2-1-5-7-4 &Flan-UL2-20B & & &4.6 &11.52 &48.47 \\
SelfAskQA &3-2-1 &Flan-UL2-20B & & &3.2 &8.53 &47.16 \\
Toolformer-Search &mixshot\_avg &Flan-PaLM-540B & & &13.1 &22.01 &74.24 \\
RARR-Top5 &mixshot\_max &Flan-PaLM-540B & & &25.0 &36.12 &80.35 \\
Toolformer-Search &5-3-6-1-4-0-2 &Flan-UL2-20B & & &7.4 &14.78 &44.98 \\
RARR &5-3-6-1-4-0-2 &Flan-UL2-20B & & &4.2 &12.98 &42.79 \\
RARR &2-1-5-7-4 &Flan-UL2-20B & & &4.8 &12.01 &40.17 \\
Non-TA-SelfAsk &3-2-1 &Flan-UL2-20B & & &3.0 &11.40 &34.06 \\
SelfAskQA &mixshot\_avg &Flan-PaLM-540B & & &12.8 &21.94 &71.91 \\
SelfAskQA-Top5 &mixshot\_max &Flan-PaLM-540B & & &12.6 &21.99 &72.05 \\
SelfAsk &2-1-5-7-4 &Flan-UL2-20B & & &2.6 &7.68 &25.76 \\
SelfAsk &5-3-6-1-4-0-2 &Flan-UL2-20B & & &2.6 &7.41 &23.14 \\
SelfAskQA &2-1-5-7-4 &Flan-UL2-20B & & &1.0 &5.35 &17.03 \\
SelfAskQA &5-3-6-1-4-0-2 &Flan-UL2-20B & & &0.8 &2.30 &11.79 \\
Interleave &mixshot\_avg &Flan-PaLM-540B & & &13.5 &21.83 &77.00 \\
Toolformer-Top5 &mixshot\_max &Flan-PaLM-540B & & &22.6 &34.53 &77.73 \\
Interleave &3-2-1 &Flan-UL2-20B & & &0.0 &0.03 &0.00 \\
Interleave &2-1-5-7-4 &Flan-UL2-20B & & & & &0.00 \\
Interleave &5-3-6-1-4-0-2 &Flan-UL2-20B & & & & &0.00 \\
RnR-Top5 &3-2-1 &Flan-UL2-20B & & &4.6 &11.45 & \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/usage.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering

\ra{1.1}
\rowcolors{1}{}{lightgray}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{lllrrrrr}\toprule
Dataset &Strategy &Model &Score &\multicolumn{3}{c}{Usage} \\\cmidrule{5-7}
& & & &3-shot &5-shot &7-shot \\\midrule
MuSiQue &SelfAsk &GPT-3 &24.1 &99.6 &99.6 &100.0 \\
MuSiQue &SelfAsk &\ULs &23.4 &37.2 &42.9 &29.3 \\
MuSiQue &SelfAsk &Flan-UL2-20B &7.7 &97.6 &75.2 &69.2 \\
MuSiQue &SelfAsk &\USs &14.8 &75.8 &92.0 &79.2 \\
MuSiQue &SelfAskQA &GPT-3 &31.3 &99.6 &99.6 &100.0 \\
MuSiQue &SelfAskQA &\ULs &21.9 &40.0 &45.0 &30.0 \\
MuSiQue &InlineQA &GPT-3 &36.6 &100.0 &100.0 &100.0 \\
MuSiQue &InlineQA &\ULs &32.4 &100.0 &100.0 &100.0 \\
MuSiQue &InlineQA &Flan-UL2-20B &17.9 &99.8 &99.8 &99.8 \\
MuSiQue &InlineQA &\USs &11.7 &100.0 &100.0 &100.0 \\
MuSiQue &Inline &GPT-3 &31.0 &100.0 &100.0 &100.0 \\
MuSiQue &Inline &\ULs &24.3 &100.0 &100.0 &100.0 \\
MuSiQue &Inline &Flan-UL2-20B &14.9 &99.2 &99.4 &99.2 \\
MuSiQue &Inline &\USs &9.4 &100.0 &100.0 &100.0 \\
MuSiQue &Check \& Fix &GPT-3 &33.0 &100.0 &100.0 &100.0 \\
MuSiQue &Check \& Fix &\ULs &33.0 &100.0 &100.0 &100.0 \\
MuSiQue &Check \& Fix &Flan-UL2-20B &11.8 &100.0 &100.0 &100.0 \\
MuSiQue &Check \& Fix &\USs &26.4 &99.8 &100.0 &100.0 \\
StrategyQA &InlineQA &GPT-3 &72.0 &100.0 &100.0 &100.0 \\
StrategyQA &InlineQA &\ULs &72.9 &100.0 &100.0 &100.0 \\
StrategyQA &InlineQA &\USs &63.3 &100.0 &100.0 &100.0 \\
StrategyQA &Inline &GPT-3 &69.4 &100.0 &100.0 &100.0 \\
StrategyQA &Inline &\ULs &73.8 &100.0 &100.0 &100.0 \\
StrategyQA &Inline &\USs &68.6 &100.0 &100.0 &100.0 \\
StrategyQA &Check \& Fix &GPT-3 &73.8 &100.0 &100.0 &100.0 \\
StrategyQA &SelfAsk &Flan-UL2-20B &25.8 &100.0 &99.6 &100.0 \\
StrategyQA &Inline &Flan-UL2-20B &52.8 &96.1 &99.1 &100.0 \\
StrategyQA &SelfAsk &\USs &67.7 &93.9 &98.7 &99.6 \\
StrategyQA &SelfAsk &GPT-3 &67.3 &93.4 &96.9 &98.7 \\
StrategyQA &SelfAskQA &GPT-3 &67.7 &83.0 &96.5 &98.7 \\
StrategyQA &Check \& Fix &Flan-UL2-20B &60.7 &65.1 &95.2 &97.4 \\
StrategyQA &Check \& Fix &\ULs &80.8 &60.3 &87.3 &95.2 \\
StrategyQA &InlineQA &Flan-UL2-20B &70.3 &52.0 &79.0 &94.3 \\
StrategyQA &Check \& Fix &\USs &71.2 &45.0 &73.4 &91.3 \\
StrategyQA &SelfAsk &\ULs &70.7 &45.0 &45.0 &79.1 \\
StrategyQA &SelfAskQA &\ULs &69.0 &24.5 &45.0 &84.0 \\
GSM8K &InlineQA &GPT-3 &52.4 &100.0 &100.0 &100.0 \\
GSM8K &Check \& Fix &\ULs &70.4 &100.0 &100.0 &100.0 \\
GSM8K &Check \& Fix &Flan-UL2-20B &25.8 &100.0 &100.0 &100.0 \\
GSM8K &Check \& Fix &\USs &44.0 &99.4 &100.0 &99.4 \\
GSM8K &Check \& Fix &GPT-3 &58.4 &98.4 &97.2 &99.2 \\
GSM8K &InlineQA &\ULs &61.4 &12.8 &17.1 &23.6 \\
GSM8K &InlineQA &Flan-UL2-20B &26.2 &0.4 &0.6 &1.0 \\
GSM8K &InlineQA &\USs &47.8 &0.0 &0.0 &0.4 \\
DROP &Check \& Fix &\USs &63.6 &100.0 &100.0 &100.0 \\
DROP &Check \& Fix &\ULs &73.6 &99.8 &99.6 &84.8 \\
DROP &InlineQA &GPT-3 &66.0 &86.4 &73.6 &78.8 \\
DROP &Check \& Fix &GPT-3 &54.4 &66.4 &63.2 &54.4 \\
DROP &InlineQA &\ULs &75.2 &49.0 &3.8 &0.0 \\
DROP &InlineQA &\USs &64.0 &24.8 &0.0 &0.0 \\
\bottomrule
\end{tabular}}
\caption{Usage statistics in percentage. Note that for some methods, tools are guaranteed to be called.}\label{tab: }
\end{table*}







==> tables/usage_prompts.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[t]\centering
% \scriptsize
\ra{1.3}
\rowcolors{1}{}{lightgray}
\footnotesize
\begin{tabular}{lrr}\toprule
Demonstrations &Usage \\\midrule
3-shot &80.9 \\
5-shot &82.5 \\
7-shot &83.7 \\
\bottomrule
\end{tabular}
\caption{Overview of average rate of tool usage across experiments. Note that RARR and Interleaving are guaranteed to use tools, so they are omitted.}\label{tab:usage-prompts}
\end{table}

